SciPhi-Chat: Training a Spatial Audio Agent for Question Answering, Dialogue, and Tool Use

Spatial audio question answering requires associating sound identities with locations and reasoning about their relations. This paper introduces SciPhi-Chat, a spatial audio agent that answers questions, conducts multi-turn dialogue, and calls tools on first-order ambisonic recordings. The accompanying MASU benchmark contains 12,000 samples across 42 task categories, the widest task coverage of any spatial model, with real recordings and simulated audio scenes. SciPhi-Chat achieves a score of 44.9%, 7.4 percentage points above the previous state-of-the-art. On the external ASA-Bench, SciPhi-Chat achieves 74.5% azimuth and 60.0% elevation accuracy, the highest among locally evaluated models. Removing reasoning supervision reduces ASA-Bench accuracy by 17.4 percentage points. All materials will be released via https://github.com/microsoft/sciphi-chat

==> figures/conversation.tex <==
% Chat inset. Coordinates and palette are inherited from the overview figure.
% Twemoji avatars (CC BY 4.0): emoji/README.txt and emoji/LICENSE-GRAPHICS.
\tikzset{
  chat/.style={rounded corners=1.5mm,line width=.4pt,inner sep=1.1mm,
    outer sep=0pt,text width=56mm,
    align=left,font=\sffamily\fontsize{6.5}{7.5}\selectfont},
  chatuser/.style={chat,draw=ovteal!25,fill=ovteal!10},
  chatagent/.style={chat,draw=ovblue!20,fill=ovblue!4},
  avatar/.style={inner sep=0pt,outer sep=0pt},
}
% Every bubble has the same width and padding. Each starts the same distance
% below the preceding bubble's actual bottom edge, regardless of text height.
\def\chatgap{1.7}
\coordinate (usercolumn) at (174.5,0);
\coordinate (agentcolumn) at (112,0);

% User messages are right-aligned; assistant messages are left-aligned.
\node[chatuser,anchor=north east] (userone) at (174.5,3) {%
  \tikz[baseline=-.5ex,x=1mm,y=1mm]{%
    \fill[ovteal] (0,-1.1) -- (0,1.1) -- (1.8,0) -- cycle;
    \foreach \x/\h in {3/.5,4/.9,5/.4,6/1.1,7/.7,8/.35}
      \draw[ovteal,line width=.55pt] (\x,-\h) -- (\x,\h);
  }\hspace{1mm}\textcolor{ovgray}{FOA audio}\hspace{2mm}
  Which source started first?};

% First response: an original reasoning span, scene fields, and the answer.
\node[chatagent,anchor=north west] (agentone)
  at ($(agentcolumn |- userone.south)+(0,\chatgap)$) {%
  \textcolor{ovgray}{\texttt{<think>}} [\ldots] It begins at just 0.2 seconds\\
  {}[\ldots] \textcolor{ovgray}{\texttt{</think>}}\\[.5mm]
  {\fontencoding{T1}\ttfamily\fontsize{6}{6.8}\selectfont
  \textcolor{ovgray}{<json>}\{\char34{}source\_count\char34{}:3,\textcolor{ovgray}{[\ldots]},\char34{}sources\char34{}:[\\
  \hspace*{1mm}\{\char34{}azimuth\char34{}:66,\char34{}elevation\char34{}:22,\textcolor{ovgray}{[\ldots]}\},\\
  \hspace*{1mm}\{\char34{}azimuth\char34{}:113,\char34{}elevation\char34{}:37,\textcolor{ovgray}{[\ldots]}\},\\
  \hspace*{1mm}\{\char34{}sound\_type\char34{}:\char34{}electric guitar\char34{},\textcolor{ovgray}{[\ldots]},\\
  \hspace*{2mm}\char34{}azimuth\char34{}:136,\char34{}elevation\char34{}:25\}]\}\textcolor{ovgray}{</json>}}\\[.5mm]
  \textcolor{ovgray}{\texttt{<answer>}} electric guitar \textcolor{ovgray}{\texttt{</answer>}}};

% The follow-up locates the guitar identified in the first answer.
\node[chatuser,anchor=north east] (usertwo)
  at ($(usercolumn |- agentone.south)+(0,\chatgap)$)
  {Which region around you is it in?};
\node[chatagent,anchor=north west] (agenttwo)
  at ($(agentcolumn |- usertwo.south)+(0,\chatgap)$)
  {\textcolor{ovgray}{\texttt{<think>}} [\ldots] The electric guitar,\\
  establishing itself from the upper back-left,\\
  provides a soft backdrop. [\ldots] \textcolor{ovgray}{\texttt{</think>}}\\[.5mm]
  \textcolor{ovgray}{\texttt{<answer>}} upper back-left \textcolor{ovgray}{\texttt{</answer>}}};

% The final exchange counts all three sources in the same recording.
\node[chatuser,anchor=north east] (userthree)
  at ($(usercolumn |- agenttwo.south)+(0,\chatgap)$)
  {How many distinct sound sources can you hear?};
\node[chatagent,anchor=north west] (agentthree)
  at ($(agentcolumn |- userthree.south)+(0,\chatgap)$)
  {\textcolor{ovgray}{\texttt{<think>}} [\ldots] I can count these sources\\
  individually without overlap; [\ldots] \textcolor{ovgray}{\texttt{</think>}}\\[.5mm]
  \textcolor{ovgray}{\texttt{<answer>}} 3 count \textcolor{ovgray}{\texttt{</answer>}}};

% Avatars use the same horizontal gap and top inset beside every bubble.
\foreach \bubble in {userone,usertwo,userthree}
  \node[avatar,anchor=north west] at ($(\bubble.north east)+(2,.7)$)
    {\includegraphics[width=4.1mm]{figures/emoji/person.pdf}};
\foreach \bubble in {agentone,agenttwo,agentthree}
  \node[avatar,anchor=north east] at ($(\bubble.north west)+(-2,.7)$)
    {\includegraphics[width=4.1mm]{figures/emoji/robot.pdf}};


==> figures/foa-waveforms.tex <==
% Real FOA excerpt, displayed in WXYZ order; stored audio remains ACN WYZX.
% This audio icon is independent of the training dialogue in the right panel.
\node[small,text=ovblue,inner sep=0mm] at (34.8,4.2) {W};
\draw[ovblue!15,line width=.25pt] (38,4.2) -- (68,4.2);
\draw[ovteal,line width=.4pt,line cap=round,line join=round] plot coordinates {
  (38.0000,4.1259) (38.1255,4.1072) (38.2510,4.0848) (38.3766,4.0793) (38.5021,4.0729) (38.6276,4.0939) (38.7531,4.1227) (38.8787,4.1696)
  (39.0042,4.2061) (39.1297,4.2430) (39.2552,4.2893) (39.3808,4.2967) (39.5063,4.3265) (39.6318,4.3420) (39.7573,4.3423) (39.8828,4.3398)
  (40.0084,4.3352) (40.1339,4.3501) (40.2594,4.3498) (40.3849,4.3595) (40.5105,4.3527) (40.6360,4.3100) (40.7615,4.2935) (40.8870,4.2343)
  (41.0126,4.1896) (41.1381,4.1185) (41.2636,4.0612) (41.3891,4.0544) (41.5146,4.1097) (41.6402,4.1971) (41.7657,4.2605) (41.8912,4.3398)
  (42.0167,4.3951) (42.1423,4.4313) (42.2678,4.4242) (42.3933,4.4190) (42.5188,4.3938) (42.6444,4.3388) (42.7699,4.3074) (42.8954,4.2450)
  (43.0209,4.1874) (43.1464,4.1389) (43.2720,4.0910) (43.3975,4.0670) (43.5230,4.0767) (43.6485,4.1246) (43.7741,4.1874) (43.8996,4.2644)
  (44.0251,4.3407) (44.1506,4.4206) (44.2762,4.4853) (44.4017,4.5364) (44.5272,4.5571) (44.6527,4.5465) (44.7782,4.5093) (44.9038,4.4543)
  (45.0293,4.3624) (45.1548,4.2501) (45.2803,4.1110) (45.4059,3.9849) (45.5314,3.8839) (45.6569,3.8186) (45.7824,3.8037) (45.9079,3.8477)
  (46.0335,3.9622) (46.1590,4.1143) (46.2845,4.2815) (46.4100,4.4193) (46.5356,4.5578) (46.6611,4.6448) (46.7866,4.6645) (46.9121,4.6539)
  (47.0377,4.6063) (47.1632,4.5381) (47.2887,4.4514) (47.4142,4.3449) (47.5397,4.2556) (47.6653,4.1589) (47.7908,4.0894) (47.9163,4.0399)
  (48.0418,4.0175) (48.1674,4.0331) (48.2929,4.0932) (48.4184,4.1715) (48.5439,4.2679) (48.6695,4.3805) (48.7950,4.4666) (48.9205,4.5685)
  (49.0460,4.6413) (49.1715,4.6830) (49.2971,4.7257) (49.4226,4.7208) (49.5481,4.7005) (49.6736,4.6526) (49.7992,4.5740) (49.9247,4.4879)
  (50.0502,4.3753) (50.1757,4.2689) (50.3013,4.1502) (50.4268,4.0269) (50.5523,3.9241) (50.6778,3.8335) (50.8033,3.7749) (50.9289,3.7578)
  (51.0544,3.8008) (51.1799,3.8927) (51.3054,4.0324) (51.4310,4.2116) (51.5565,4.4045) (51.6820,4.5743) (51.8075,4.7157) (51.9331,4.8334)
  (52.0586,4.8661) (52.1841,4.8606) (52.3096,4.7613) (52.4351,4.6157) (52.5607,4.4827) (52.6862,4.3268) (52.8117,4.1628) (52.9372,4.0192)
  (53.0628,3.8836) (53.1883,3.8354) (53.3138,3.7804) (53.4393,3.7629) (53.5649,3.8419) (53.6904,3.9664) (53.8159,4.1524) (53.9414,4.3307)
  (54.0669,4.4954) (54.1925,4.5413) (54.3180,4.5507) (54.4435,4.5400) (54.5690,4.4983) (54.6946,4.5002) (54.8201,4.4536) (54.9456,4.3378)
  (55.0711,4.2382) (55.1967,4.1162) (55.3222,3.9739) (55.4477,3.8419) (55.5732,3.8309) (55.6987,3.8073) (55.8243,3.8283) (55.9498,3.9198)
  (56.0753,3.9503) (56.2008,3.9538) (56.3264,3.9739) (56.4519,4.0602) (56.5774,4.0596) (56.7029,4.1893) (56.8285,4.2961) (56.9540,4.3925)
  (57.0795,4.4882) (57.2050,4.4789) (57.3305,4.4866) (57.4561,4.3854) (57.5816,4.3355) (57.7071,4.2485) (57.8326,4.1770) (57.9582,4.0150)
  (58.0837,3.9169) (58.2092,3.7814) (58.3347,3.6471) (58.4603,3.6863) (58.5858,3.7432) (58.7113,3.7976) (58.8368,3.8121) (58.9623,3.8875)
  (59.0879,4.0214) (59.2134,4.1919) (59.3389,4.2932) (59.4644,4.3915) (59.5900,4.4811) (59.7155,4.5099) (59.8410,4.5646) (59.9665,4.5536)
  (60.0921,4.4944) (60.2176,4.3478) (60.3431,4.3165) (60.4686,4.2605) (60.5941,4.1670) (60.7197,4.0402) (60.8452,3.9279) (60.9707,3.8771)
  (61.0962,3.8574) (61.2218,3.9347) (61.3473,3.9962) (61.4728,4.0305) (61.5983,3.9852) (61.7238,4.0415) (61.8494,4.1437) (61.9749,4.2288)
  (62.1004,4.3459) (62.2259,4.4310) (62.3515,4.4653) (62.4770,4.5148) (62.6025,4.6639) (62.7280,4.6422) (62.8536,4.6063) (62.9791,4.5636)
  (63.1046,4.4837) (63.2301,4.4326) (63.3556,4.3375) (63.4812,4.2181) (63.6067,4.0641) (63.7322,3.9978) (63.8577,3.9955) (63.9833,4.0531)
  (64.1088,3.9435) (64.2343,3.9260) (64.3598,3.9755) (64.4854,4.0984) (64.6109,4.3559) (64.7364,4.5714) (64.8619,4.6904) (64.9874,4.7024)
  (65.1130,4.8127) (65.2385,4.8509) (65.3640,4.8800) (65.4895,4.8428) (65.6151,4.7464) (65.7406,4.5332) (65.8661,4.3611) (65.9916,4.2446)
  (66.1172,4.1275) (66.2427,3.9836) (66.3682,3.8674) (66.4937,3.8771) (66.6192,3.9684) (66.7448,4.0072) (66.8703,4.0392) (66.9958,3.9968)
  (67.1213,4.0260) (67.2469,4.2624) (67.3724,4.5131) (67.4979,4.5565) (67.6234,4.4976) (67.7490,4.4501) (67.8745,4.4565) (68.0000,4.6024)
};
\node[small,text=ovblue,inner sep=0mm] at (34.8,6.05) {X};
\draw[ovblue!15,line width=.25pt] (38,6.05) -- (68,6.05);
\draw[ovteal,line width=.4pt,line cap=round,line join=round] plot coordinates {
  (38.0000,6.0613) (38.1255,6.0697) (38.2510,6.0730) (38.3766,6.0697) (38.5021,6.0581) (38.6276,6.0574) (38.7531,6.0500) (38.8787,6.0426)
  (39.0042,6.0400) (39.1297,6.0461) (39.2552,6.0659) (39.3808,6.0788) (39.5063,6.0840) (39.6318,6.0950) (39.7573,6.1073) (39.8828,6.1089)
  (40.0084,6.0979) (40.1339,6.0943) (40.2594,6.0895) (40.3849,6.0946) (40.5105,6.0898) (40.6360,6.0710) (40.7615,6.0506) (40.8870,6.0270)
  (41.0126,6.0067) (41.1381,5.9759) (41.2636,5.9565) (41.3891,5.9520) (41.5146,5.9659) (41.6402,5.9837) (41.7657,5.9995) (41.8912,6.0176)
  (42.0167,6.0319) (42.1423,6.0348) (42.2678,6.0393) (42.3933,6.0374) (42.5188,6.0270) (42.6444,6.0248) (42.7699,6.0209) (42.8954,6.0128)
  (43.0209,6.0141) (43.1464,6.0157) (43.2720,6.0118) (43.3975,6.0002) (43.5230,5.9639) (43.6485,5.9352) (43.7741,5.9151) (43.8996,5.9009)
  (44.0251,5.8999) (44.1506,5.9251) (44.2762,5.9782) (44.4017,6.0406) (44.5272,6.1056) (44.6527,6.1681) (44.7782,6.2017) (44.9038,6.2208)
  (45.0293,6.2001) (45.1548,6.1635) (45.2803,6.1137) (45.4059,6.0752) (45.5314,6.0396) (45.6569,6.0122) (45.7824,5.9924) (45.9079,5.9914)
  (46.0335,6.0041) (46.1590,6.0180) (46.2845,6.0306) (46.4100,6.0503) (46.5356,6.0746) (46.6611,6.0950) (46.7866,6.1008) (46.9121,6.1034)
  (47.0377,6.1179) (47.1632,6.1318) (47.2887,6.1441) (47.4142,6.1409) (47.5397,6.1373) (47.6653,6.1173) (47.7908,6.0794) (47.9163,6.0280)
  (48.0418,5.9662) (48.1674,5.9177) (48.2929,5.8860) (48.4184,5.8808) (48.5439,5.8818) (48.6695,5.9183) (48.7950,5.9672) (48.9205,6.0387)
  (49.0460,6.0995) (49.1715,6.1218) (49.2971,6.1464) (49.4226,6.1422) (49.5481,6.1312) (49.6736,6.1108) (49.7992,6.0772) (49.9247,6.0642)
  (50.0502,6.0536) (50.1757,6.0448) (50.3013,6.0251) (50.4268,6.0079) (50.5523,5.9830) (50.6778,5.9555) (50.8033,5.9420) (50.9289,5.9255)
  (51.0544,5.9310) (51.1799,5.9432) (51.3054,5.9620) (51.4310,5.9898) (51.5565,6.0199) (51.6820,6.0500) (51.8075,6.0849) (51.9331,6.1241)
  (52.0586,6.1509) (52.1841,6.1836) (52.3096,6.1982) (52.4351,6.1936) (52.5607,6.1881) (52.6862,6.1733) (52.8117,6.1535) (52.9372,6.1299)
  (53.0628,6.0846) (53.1883,6.0532) (53.3138,6.0057) (53.4393,5.9529) (53.5649,5.9154) (53.6904,5.8886) (53.8159,5.9070) (53.9414,5.9361)
  (54.0669,5.9898) (54.1925,6.0270) (54.3180,6.0840) (54.4435,6.1383) (54.5690,6.1723) (54.6946,6.2011) (54.8201,6.2014) (54.9456,6.1784)
  (55.0711,6.1506) (55.1967,6.1089) (55.3222,6.0733) (55.4477,6.0613) (55.5732,6.0730) (55.6987,6.0338) (55.8243,5.9992) (55.9498,5.9313)
  (56.0753,5.9009) (56.2008,5.8643) (56.3264,5.8504) (56.4519,5.8617) (56.5774,5.8753) (56.7029,5.9154) (56.8285,5.9808) (56.9540,6.0458)
  (57.0795,6.0739) (57.2050,6.0739) (57.3305,6.1393) (57.4561,6.1590) (57.5816,6.2008) (57.7071,6.2176) (57.8326,6.2247) (57.9582,6.1995)
  (58.0837,6.1538) (58.2092,6.1082) (58.3347,6.0361) (58.4603,6.0089) (58.5858,5.9766) (58.7113,6.0060) (58.8368,5.9439) (58.9623,5.8779)
  (59.0879,5.8339) (59.2134,5.8352) (59.3389,5.8701) (59.4644,5.9025) (59.5900,5.9866) (59.7155,6.0494) (59.8410,6.1289) (59.9665,6.1843)
  (60.0921,6.2211) (60.2176,6.1885) (60.3431,6.1982) (60.4686,6.1784) (60.5941,6.1289) (60.7197,6.1053) (60.8452,6.0316) (60.9707,6.0322)
  (61.0962,5.9759) (61.2218,5.9445) (61.3473,5.9568) (61.4728,5.9300) (61.5983,5.8756) (61.7238,5.8491) (61.8494,5.8449) (61.9749,5.8420)
  (62.1004,5.9452) (62.2259,5.9840) (62.3515,6.0251) (62.4770,6.0817) (62.6025,6.1781) (62.7280,6.2532) (62.8536,6.2684) (62.9791,6.2574)
  (63.1046,6.2237) (63.2301,6.1988) (63.3556,6.1826) (63.4812,6.1593) (63.6067,6.0959) (63.7322,6.0380) (63.8577,5.9808) (63.9833,5.9481)
  (64.1088,5.9077) (64.2343,5.8617) (64.3598,5.8404) (64.4854,5.8116) (64.6109,5.8501) (64.7364,5.9157) (64.8619,5.9555) (64.9874,5.9811)
  (65.1130,6.0756) (65.2385,6.1493) (65.3640,6.2431) (65.4895,6.2933) (65.6151,6.2884) (65.7406,6.2567) (65.8661,6.1509) (65.9916,6.1208)
  (66.1172,6.0992) (66.2427,6.0594) (66.3682,5.9889) (66.4937,5.9788) (66.6192,5.9529) (66.7448,5.9248) (66.8703,5.9377) (66.9958,5.8721)
  (67.1213,5.8510) (67.2469,5.8420) (67.3724,5.8999) (67.4979,5.9633) (67.6234,6.0005) (67.7490,6.0649) (67.8745,6.1176) (68.0000,6.1771)
};
\node[small,text=ovblue,inner sep=0mm] at (34.8,7.95) {Y};
\draw[ovblue!15,line width=.25pt] (38,7.95) -- (68,7.95);
\draw[ovteal,line width=.4pt,line cap=round,line join=round] plot coordinates {
  (38.0000,8.0115) (38.1255,8.0251) (38.2510,8.0386) (38.3766,8.0509) (38.5021,8.0461) (38.6276,8.0386) (38.7531,8.0196) (38.8787,7.9956)
  (39.0042,7.9701) (39.1297,7.9435) (39.2552,7.9293) (39.3808,7.9157) (39.5063,7.9157) (39.6318,7.9186) (39.7573,7.9338) (39.8828,7.9312)
  (40.0084,7.9322) (40.1339,7.9358) (40.2594,7.9461) (40.3849,7.9555) (40.5105,7.9558) (40.6360,7.9730) (40.7615,7.9963) (40.8870,8.0124)
  (41.0126,8.0364) (41.1381,8.0532) (41.2636,8.0597) (41.3891,8.0545) (41.5146,8.0331) (41.6402,7.9979) (41.7657,7.9604) (41.8912,7.9312)
  (42.0167,7.8973) (42.1423,7.8798) (42.2678,7.8639) (42.3933,7.8529) (42.5188,7.8584) (42.6444,7.8711) (42.7699,7.8969) (42.8954,7.9244)
  (43.0209,7.9561) (43.1464,7.9824) (43.2720,8.0111) (43.3975,8.0403) (43.5230,8.0471) (43.6485,8.0451) (43.7741,8.0380) (43.8996,8.0199)
  (44.0251,8.0011) (44.1506,7.9671) (44.2762,7.9429) (44.4017,7.9209) (44.5272,7.9050) (44.6527,7.8859) (44.7782,7.8568) (44.9038,7.8394)
  (45.0293,7.8339) (45.1548,7.8429) (45.2803,7.8652) (45.4059,7.8982) (45.5314,7.9416) (45.6569,7.9804) (45.7824,8.0037) (45.9079,8.0105)
  (46.0335,8.0050) (46.1590,7.9921) (46.2845,7.9746) (46.4100,7.9497) (46.5356,7.9316) (46.6611,7.9186) (46.7866,7.9251) (46.9121,7.9309)
  (47.0377,7.9458) (47.1632,7.9604) (47.2887,7.9710) (47.4142,7.9791) (47.5397,7.9895) (47.6653,7.9911) (47.7908,7.9891) (47.9163,7.9836)
  (48.0418,7.9684) (48.1674,7.9510) (48.2929,7.9270) (48.4184,7.9073) (48.5439,7.8944) (48.6695,7.8850) (48.7950,7.8892) (48.9205,7.8995)
  (49.0460,7.9277) (49.1715,7.9513) (49.2971,7.9701) (49.4226,7.9849) (49.5481,7.9966) (49.6736,7.9943) (49.7992,7.9769) (49.9247,7.9581)
  (50.0502,7.9351) (50.1757,7.9293) (50.3013,7.9257) (50.4268,7.9244) (50.5523,7.9290) (50.6778,7.9442) (50.8033,7.9597) (50.9289,7.9568)
  (51.0544,7.9545) (51.1799,7.9610) (51.3054,7.9620) (51.4310,7.9665) (51.5565,7.9671) (51.6820,7.9817) (51.8075,7.9937) (51.9331,8.0034)
  (52.0586,8.0001) (52.1841,7.9953) (52.3096,7.9811) (52.4351,7.9649) (52.5607,7.9371) (52.6862,7.9189) (52.8117,7.9028) (52.9372,7.9008)
  (53.0628,7.9128) (53.1883,7.9319) (53.3138,7.9681) (53.4393,8.0037) (53.5649,8.0299) (53.6904,8.0412) (53.8159,8.0380) (53.9414,8.0247)
  (54.0669,8.0108) (54.1925,8.0021) (54.3180,8.0011) (54.4435,7.9817) (54.5690,7.9477) (54.6946,7.9086) (54.8201,7.8707) (54.9456,7.8559)
  (55.0711,7.8442) (55.1967,7.8300) (55.3222,7.8284) (55.4477,7.8403) (55.5732,7.8449) (55.6987,7.8698) (55.8243,7.8921) (55.9498,7.9160)
  (56.0753,7.9769) (56.2008,8.0289) (56.3264,8.0454) (56.4519,8.0522) (56.5774,8.0791) (56.7029,8.0752) (56.8285,8.0639) (56.9540,8.0215)
  (57.0795,7.9568) (57.2050,7.9128) (57.3305,7.8575) (57.4561,7.8536) (57.5816,7.8429) (57.7071,7.8390) (57.8326,7.8494) (57.9582,7.8775)
  (58.0837,7.8843) (58.2092,7.9109) (58.3347,7.9484) (58.4603,7.9859) (58.5858,8.0131) (58.7113,8.0606) (58.8368,8.0972) (58.9623,8.0920)
  (59.0879,8.0616) (59.2134,8.0623) (59.3389,8.0370) (59.4644,8.0027) (59.5900,7.9794) (59.7155,7.9649) (59.8410,7.9341) (59.9665,7.9274)
  (60.0921,7.8963) (60.2176,7.8921) (60.3431,7.8772) (60.4686,7.8665) (60.5941,7.8827) (60.7197,7.8889) (60.8452,7.9186) (60.9707,7.9261)
  (61.0962,7.9193) (61.2218,7.8953) (61.3473,7.9367) (61.4728,7.9963) (61.5983,8.0597) (61.7238,8.0810) (61.8494,8.0623) (61.9749,8.0370)
  (62.1004,8.0111) (62.2259,8.0318) (62.3515,8.0069) (62.4770,7.9814) (62.6025,7.9694) (62.7280,7.9358) (62.8536,7.8918) (62.9791,7.8594)
  (63.1046,7.8407) (63.2301,7.8264) (63.3556,7.8416) (63.4812,7.8526) (63.6067,7.8824) (63.7322,7.8853) (63.8577,7.9015) (63.9833,7.9578)
  (64.1088,8.0053) (64.2343,8.0568) (64.3598,8.1037) (64.4854,8.1143) (64.6109,8.0700) (64.7364,8.0710) (64.8619,8.0619) (64.9874,8.0742)
  (65.1130,8.0367) (65.2385,7.9950) (65.3640,7.9413) (65.4895,7.8866) (65.6151,7.8827) (65.7406,7.8918) (65.8661,7.8782) (65.9916,7.8193)
  (66.1172,7.8064) (66.2427,7.8022) (66.3682,7.7925) (66.4937,7.8174) (66.6192,7.8416) (66.7448,7.8834) (66.8703,7.9231) (66.9958,7.9807)
  (67.1213,8.0108) (67.2469,8.0079) (67.3724,8.0218) (67.4979,8.0713) (67.6234,8.1069) (67.7490,8.0804) (67.8745,8.0218) (68.0000,7.9325)
};
\node[small,text=ovblue,inner sep=0mm] at (34.8,9.8) {Z};
\draw[ovblue!15,line width=.25pt] (38,9.8) -- (68,9.8);
\draw[ovteal,line width=.4pt,line cap=round,line join=round] plot coordinates {
  (38.0000,9.8531) (38.1255,9.8828) (38.2510,9.8815) (38.3766,9.8890) (38.5021,9.8844) (38.6276,9.8663) (38.7531,9.8469) (38.8787,9.8252)
  (39.0042,9.8168) (39.1297,9.7945) (39.2552,9.7657) (39.3808,9.7340) (39.5063,9.7110) (39.6318,9.6894) (39.7573,9.6706) (39.8828,9.6583)
  (40.0084,9.6590) (40.1339,9.6709) (40.2594,9.6884) (40.3849,9.7165) (40.5105,9.7405) (40.6360,9.7951) (40.7615,9.8446) (40.8870,9.9025)
  (41.0126,9.9569) (41.1381,10.0035) (41.2636,10.0320) (41.3891,10.0261) (41.5146,9.9747) (41.6402,9.8977) (41.7657,9.8201) (41.8912,9.7466)
  (42.0167,9.6926) (42.1423,9.6632) (42.2678,9.6599) (42.3933,9.6810) (42.5188,9.7107) (42.6444,9.7622) (42.7699,9.8003) (42.8954,9.8440)
  (43.0209,9.8815) (43.1464,9.9132) (43.2720,9.9320) (43.3975,9.9462) (43.5230,9.9488) (43.6485,9.9488) (43.7741,9.9472) (43.8996,9.9414)
  (44.0251,9.9372) (44.1506,9.9249) (44.2762,9.9126) (44.4017,9.8954) (44.5272,9.8809) (44.6527,9.8789) (44.7782,9.8996) (44.9038,9.9372)
  (45.0293,9.9902) (45.1548,10.0559) (45.2803,10.1070) (45.4059,10.1565) (45.5314,10.1487) (45.6569,10.1222) (45.7824,10.0627) (45.9079,9.9488)
  (46.0335,9.8116) (46.1590,9.6871) (46.2845,9.5920) (46.4100,9.5412) (46.5356,9.5273) (46.6611,9.5409) (46.7866,9.5968) (46.9121,9.6797)
  (47.0377,9.7618) (47.1632,9.8061) (47.2887,9.8653) (47.4142,9.9022) (47.5397,9.9194) (47.6653,9.9242) (47.7908,9.8971) (47.9163,9.8699)
  (48.0418,9.8220) (48.1674,9.7744) (48.2929,9.7178) (48.4184,9.6680) (48.5439,9.6188) (48.6695,9.5674) (48.7950,9.5406) (48.9205,9.5046)
  (49.0460,9.4801) (49.1715,9.4765) (49.2971,9.4885) (49.4226,9.5363) (49.5481,9.5933) (49.6736,9.6590) (49.7992,9.7317) (49.9247,9.8084)
  (50.0502,9.8728) (50.1757,9.9171) (50.3013,9.9514) (50.4268,9.9731) (50.5523,9.9860) (50.6778,9.9837) (50.8033,9.9692) (50.9289,9.9339)
  (51.0544,9.8773) (51.1799,9.8084) (51.3054,9.7317) (51.4310,9.6395) (51.5565,9.5532) (51.6820,9.4878) (51.8075,9.4668) (51.9331,9.4726)
  (52.0586,9.5299) (52.1841,9.6240) (52.3096,9.7495) (52.4351,9.8783) (52.5607,9.9614) (52.6862,10.0232) (52.8117,10.0620) (52.9372,10.0782)
  (53.0628,10.0811) (53.1883,10.0488) (53.3138,10.0391) (53.4393,10.0539) (53.5649,10.0155) (53.6904,9.9757) (53.8159,9.8925) (53.9414,9.8440)
  (54.0669,9.8113) (54.1925,9.8754) (54.3180,9.9527) (54.4435,9.9996) (54.5690,10.0093) (54.6946,9.9708) (54.8201,9.9359) (54.9456,9.9349)
  (55.0711,9.9116) (55.1967,9.8854) (55.3222,9.8835) (55.4477,9.9242) (55.5732,9.8443) (55.6987,9.8003) (55.8243,9.7987) (55.9498,9.8168)
  (56.0753,9.9038) (56.2008,9.9880) (56.3264,10.0501) (56.4519,10.0258) (56.5774,10.0627) (56.7029,9.9951) (56.8285,9.9213) (56.9540,9.8162)
  (57.0795,9.7266) (57.2050,9.7120) (57.3305,9.6437) (57.4561,9.6363) (57.5816,9.5975) (57.7071,9.5606) (57.8326,9.5363) (57.9582,9.6408)
  (58.0837,9.6761) (58.2092,9.7055) (58.3347,9.7880) (58.4603,9.7130) (58.5858,9.7036) (58.7113,9.7178) (58.8368,9.7673) (58.9623,9.7919)
  (59.0879,9.8168) (59.2134,9.7227) (59.3389,9.7253) (59.4644,9.7017) (59.5900,9.6884) (59.7155,9.6916) (59.8410,9.6638) (59.9665,9.6188)
  (60.0921,9.6505) (60.2176,9.6716) (60.3431,9.5794) (60.4686,9.6221) (60.5941,9.6305) (60.7197,9.6852) (60.8452,9.7667) (60.9707,9.7437)
  (61.0962,9.7049) (61.2218,9.6955) (61.3473,9.7253) (61.4728,9.7764) (61.5983,9.9258) (61.7238,9.9553) (61.8494,9.9792) (61.9749,9.9863)
  (62.1004,9.8857) (62.2259,9.8563) (62.3515,9.8375) (62.4770,9.7560) (62.6025,9.7292) (62.7280,9.7146) (62.8536,9.6117) (62.9791,9.6166)
  (63.1046,9.6538) (63.2301,9.6991) (63.3556,9.8149) (63.4812,9.9245) (63.6067,9.9747) (63.7322,9.9922) (63.8577,9.9275) (63.9833,9.8207)
  (64.1088,9.9407) (64.2343,9.9533) (64.3598,9.9928) (64.4854,9.9957) (64.6109,9.8598) (64.7364,9.7689) (64.8619,9.7777) (64.9874,9.8142)
  (65.1130,9.7861) (65.2385,9.8679) (65.3640,9.8168) (65.4895,9.8272) (65.6151,9.8366) (65.7406,9.8430) (65.8661,9.9368) (65.9916,9.9786)
  (66.1172,9.9737) (66.2427,9.9705) (66.3682,9.9579) (66.4937,9.8136) (66.6192,9.8204) (66.7448,9.8556) (66.8703,9.9006) (66.9958,10.0151)
  (67.1213,10.0769) (67.2469,9.9650) (67.3724,9.9178) (67.4979,9.9462) (67.6234,9.9847) (67.7490,10.0763) (67.8745,9.9685) (68.0000,9.8207)
};

